Black Hole Metric: Overcoming the PageRank Normalization Problem

In network science, there is often the need to sort the graph nodes. While the sorting strategy may be different, in general sorting is performed by exploiting the network structure. In particular, the metric PageRank has been used in the past decade in different ways to produce a ranking based on how many neighbors point to a specific node. PageRank is simple, easy to compute and effective in many applications, however it comes with a price: as PageRank is an application of the random walker, the arc weights need to be normalized. This normalization, while necessary, introduces a series of unwanted side-effects. In this paper, we propose a generalization of PageRank named Black Hole Metric which mitigates the problem. We devise a scenario in which the side-effects are particularily impactful on the ranking, test the new metric in both real and synthetic networks, and show the results.

==> meaning.tex <==
\section[Meaning]{Meaning of black hole} \label{s:meaning}
Now that we've obtained pagerank values for each node, we may simply discard
the black hole pagerank and sort the remaining nodes, but there's more than
that: the black hole pagerank can be used as a way to gauge the global
waryness of the network. The higher its value, the less nodes trust each
other. We may define the \textit{waryness} of the network as a function of
the unassigned trust and the black hole pagerank:
\[
W = \sqrt{\frac{p_b}{\max{P}} \cdot \sum_{k=1}^N \frac{b_k + s_k}{N}}
\]
$W$ has several properties:
\begin{enumerate}
	\item It is dependant on the network topology.
	\item It is dependant on the weight assignements.
	\item $0 \le W \le 1$.
	\item $W = 0 \Leftrightarrow B = \zeromat{N}{1}$ and $p_b = 0$.
        \label{itm:max-trust}
	\item $W = 1 \Leftrightarrow B = \onemat{N}{1}$ and $p_b = \max{P}$.
        \label{itm:min-trust}
\end{enumerate}
property \ref{itm:max-trust} is satisfied when every node in the network
completely trust its neighbors, while property \ref{itm:min-trust} is
satisfied when every node in the network places no trust in its neighbors
(virtually equivalent to each node being a sink). Since its value is
normalized to the network parameters, the waryness of two different networks
can be compared.



